EDD: Efficient Differentiable DNN Architecture and Implementation Co-search for Embedded AI Solutions

High quality AI solutions require joint optimization of AI algorithms and their hardware implementations. In this work, we are the first to propose a fully simultaneous, efficient differentiable DNN architecture and implementation co-search (EDD) methodology. We formulate the co-search problem by fusing DNN search variables and hardware implementation variables into one solution space, and maximize both algorithm accuracy and hardware implementation quality. The formulation is differentiable with respect to the fused variables, so that gradient descent algorithm can be applied to greatly reduce the search time. The formulation is also applicable for various devices with different objectives. In the experiments, we demonstrate the effectiveness of our EDD methodology by searching for three representative DNNs, targeting low-latency GPU implementation and FPGA implementations with both recursive and pipelined architectures. Each model produced by EDD achieves similar accuracy as the best existing DNN models searched by neural architecture search (NAS) methods on ImageNet, but with superior performance obtained within 12 GPU-hour searches. Our DNN targeting GPU is 1.40x faster than the state-of-the-art solution reported in Proxyless, and our DNN targeting FPGA delivers 1.45x higher throughput than the state-of-the-art solution reported in DNNBuilder.

==> comments.tex <==




Weaknesses
---------------------------------------------------------------------------
- The paper does not provide enough background into the techniques that it references.
- It is difficult to understand what the innovation is.
- The proposed techniques appear to be obvious or incremental.

* This paper jumps into many details without explaining the big picture of what the techniques aim to accomplish. As a result, it is very difficult for the reader to understand the motivation of each choice and follow what is going on in each section of the paper.
 
* Neural Architecture Search (NAS) – The paper does not sufficiently or clearly explain how NAS works and how NAS is different than standard hyperparameter search. Hyperparameter search and optimization tools have been around for a long time. Many people have used these tools to automatically generate networks while including the number of operations as a loss function. How does NAS compare to these other hyperparameter search tools and why is it interesting in particular?

* Differentiable – Although “Differentiable” is in the title of the paper, it never explains why it matters if aspects of the architecture are differentiable. I can guess that the hyperparameter search tool uses a type of stochastic gradient descent, but that is never explained. It is also not explained why no one has thought of doing this before, or why it’s difficult, considering people in the past have done hyperparameter search and have included the number of operations as a constraint.

* Levels – In Section 3.2, the paper explains four levels that exist in the implementation. It is never explained what “levels” means. It’s like describing the contents of each of four floors of a building but never explaining what a “floor” in a building means to someone who doesn’t already know. Maybe this is obvious if the reader is already familiar with NAS, but I am not.

* Resource – This term is used on all pages (1-6), but it is never fully defined. There is some color added to the term on Page 4 when describing the use of accelerators. But it is never clearly defined what the authors mean with that word.

* The EfficientNet paper, which also has “Efficient” in the title, similarly attempts to optimize the number of parameters as well as the number of operations in neural networks. EfficientNet is also performing a search on MBConv-based networks. It is not clear why EfficientNet is not referred to or compared against in this paper since the goals are so similar.

* The author should be careful about how they use the word “performance” since in the machine learning community it is often used to mean accuracy. It would be better to say latency, throughput, energy, or whatever is specifically meant at the time. On page 1, “performance” is used 6 times before it is defined as “latency, throughput, or energy”.

* It is not clear what is innovative about the latency cost function (14). It appears to be calculating the number of operations… this is the most obvious and simplest way of doing it.




- Implementation formulation with levels1-4 could be elaborated in a simpler way. 
- Experimental section should be elaborated to give more details on training set size, how the number of channels in initial DNN architecture is chosen.




* In recursive implementation M-IP instantiations are used, which will be recursively used for N blocks and this will lead to inefficiency in the block where all the M layers are not used. 
* What are the final searched FPGA implementation parameters for EDD-Net2 and EDD-Net3? 
* What is the training subset size (1.28M/10 ??)
* Each chosen model is trained for 50 epochs ? What is the training set up (learning rate, schedule, optimizer, number of epochs) for the final chosen model architectures. More details on the training process and time taken for searching for each of the solutions would help the researchers in the area. 
* How is the number of channels per layer in the initial DNN chosen? That doesn’t seem to be a searched parameter. What are the bounds for the M and N? 
* Fig.4: Showing the final bit-widths of each layer would help understand if there is any trend in the bit-widths (e.g. more bit-widths in initial layers than later layers)

* The implementation cost function for latency might be oversimplified.
* The generated design parameters can only be used as a general outline for accelerator design.
* The cost function for latency might be oversimplified. It is only relating the cost to the size of the networks, which is only considering the entire hardware is fully used without any stall in the computation process. This scenario is too ideal for most DNN computations. 
* Also, the generated hardware parameters could only be used as a rough estimate for the accelerator design. For most of the accelerator design, a modular design with those generated rough estimate usually do not provide the best performance. In general, promising results for the innovations and would like to see more results following this paper.

* It is not clear how much of the benefits seen are due to the specific approach followed in the paper, rather than of applying a general NAS on the given problems

* While the results seem to indicate that the search gives a better implementation / network architecture solution than previously known, it is not clear from the paper how much of the benefit was due specifically to the method employed.  

* Since there is a multi-stage process: first fix some implementation details and train weights, then optimize Theta, Phi and I and again retrain, it would be important to see what happens at the intermediate stage before the implementation search and to confirm that the presented approach actually guided the search for a better solution. There are many heuristic approximations the authors make, and the results presented are not broad enough to make it clear that the approach will perform well in general.

